ModSRAM: Algorithm-Hardware Co-Design for Large Number Modular Multiplication in SRAM

Elliptic curve cryptography (ECC) is widely used in security applications such as public key cryptography (PKC) and zero-knowledge proofs (ZKP). ECC is composed of modular arithmetic, where modular multiplication takes most of the processing time. Computational complexity and memory constraints of ECC limit the performance. Therefore, hardware acceleration on ECC is an active field of research. Processing-in-memory (PIM) is a promising approach to tackle this problem. In this work, we design ModSRAM, the first 8T SRAM PIM architecture to compute large-number modular multiplication efficiently. In addition, we propose R4CSA-LUT, a new algorithm that reduces the cycles for an interleaved algorithm and eliminates carry propagation for addition based on look-up tables (LUT). ModSRAM is co-designed with R4CSA-LUT to support modular multiplication and data reuse in memory with 52% cycle reduction compared to prior works with only 32% area overhead.

==> fig_tex/fig_cmp.tex <==
\begin{figure}[b] 
  \centering
  \includegraphics[scale=0.4]{figures/cmp.png}
  \caption{logic-SA module for all 2 \& 3 input logic.}
  \label{fig:cmp}
  \Description{A block diagram to show logic-SA.}
\end{figure}

==> fig_tex/fig_ntt_eval.tex <==
\begin{figure}[t] 
  \centering
  \includegraphics[width=\linewidth]{figures/ZKP_OPERATIONS_NTT_MSM.pdf}
  \vspace{-20pt}
  \caption{Illustration of the scale of operations in ZKP components: NTT, INTT and MSM.}
  \label{fig: ntt-eval}
  \Description{Demonstration of the scale of operations in ZKP Components: NTT, INTT, and MSM.}
\end{figure}

==> tab_tex/tab_ZKP_MSM_NTT_operations.tex <==
\begin{table} \small
  \caption{Number of operations in ZKP: NTT and MSM} \label{tab:ZKP-NTT-MSM}
  \begin{tabular}{ccc}
    \toprule
    Operation & NTT~\cite{PNTT} & MSM~\cite{PipeZK} \\
    \midrule
    Modular Multiplications & 3936384 & 7864320 \\
    Memory Accesses & 1214016 & 131072 \\
    Register Writes & 108933112 & 478150656  \\
  \bottomrule
  \end{tabular}
\end{table}
